The Dynamic ECME Algorithm

The ECME algorithm has proven to be an effective way of accelerating the EM algorithm for many problems. Recognising the limitation of using prefixed acceleration subspace in ECME, we propose the new Dynamic ECME (DECME) algorithm which allows the acceleration subspace to be chosen dynamically. Our investigation of an inefficient special case of DECME, the classical Successive Overrelaxation (SOR) method, leads to an efficient, simple, and widely applicable DECME implementation, called DECME_v1. The fast convergence of DECME_v1 is established by the theoretical result that, in a small neighbourhood of the maximum likelihood estimate (MLE), DECME_v1 is equivalent to a conjugate direction method. Numerical results show that DECME_v1 and its two variants are very stable and often converge faster than EM by a factor of one hundred in terms of number of iterations and a factor of thirty in terms of CPU time when EM is very slow.

==> 00README.tex <==
nohypertex


==> INSTALL <==
THE BBOLD SYMBOL FONT

6 APRIL 1994

This distribution contains the bbold symbol font:

   INSTALL      bbgreeku.mf  bbold.dtx    bbold17.mf   bbold8.mf    
   README       bbligs.mf    bbold.mf     bbold5.mf    bbold9.mf
   bbbase.mf    bblower.mf   bbold10.mf   bbold6.mf    bbparams.mf
   bbgreekl.mf  bbnum.mf     bbold12.mf   bbold7.mf    bbpunc.mf
   bbupper.mf

To install the fonts, you should:

 * run METAFONT on the fonts, for example under Unix you say:

      mf "\mode=localfont; input bbold5;"
      mf "\mode=localfont; input bbold6;"
      mf "\mode=localfont; input bbold7;"
      mf "\mode=localfont; input bbold8;"
      mf "\mode=localfont; input bbold9;"
      mf "\mode=localfont; input bbold12;"
      mf "\mode=localfont; input bbold17;"

 * move bbold*.tfm into a TeX font metrics directory

 * move bbold*.*pk into a TeX bitmaps directory

If you want to use the bbold font in LaTeX2e, you should:

 * run LaTeX2e on bbold.dtx

 * move bbold.sty and Ubbold.fd into a TeX inputs directory

 * read the documentation in bbold.dvi

This file should only be distributed as part of the bbold
distribution.

Copyright 1994 Alan Jeffrey

